Exploring the Impact of Emotional Voice Integration in Sign-to-Speech Translators for Deaf-to-Hearing Communication

Emotional voice communication plays a crucial role in effective daily interactions. Deaf and hard-of-hearing (DHH) individuals often rely on facial expressions to supplement sign language to convey emotions, as the use of voice is limited. However, in American Sign Language (ASL), these facial expressions serve not only emotional purposes but also as linguistic markers, altering sign meanings and often confusing non-signers when interpreting a signer's emotional state. Most existing ASL translation technologies focus solely on signs, neglecting the role of emotional facial expressions in the translated output (e.g., text, voice). This paper present studies which 1) confirmed the challenges for non-signers of interpreting emotions from facial expressions in ASL communication, of facial expressions, and 2) how integrating emotional voices into translation systems can enhance hearing individuals' comprehension of a signer's emotions. An online survey conducted with 45 hearing participants (Non-ASL Signers) revealed that they frequently misinterpret signers' emotions when emotional and linguistic facial expressions are used simultaneously. The findings indicate that incorporating emotional voice into translation systems significantly improves the recognition of signers' emotions by 32%. Additionally, further research involving 6 DHH participants discusses design considerations for the emotional voice feature from both perspectives, emphasizing the importance of integrating emotional voices in translation systems to bridge communication gaps between DHH and hearing communities.

==> document/01_introduction.tex <==
\section{Introduction}



Sign language translation systems convert sign language into text or speech, helping hearing, non-signing individuals understand signed languages, bridging the communication gap between hearing people and signers \cite{grover2021sign, dreuw2010signspeak, fang2017deepasl}. However, current translation systems \cite{san2008speech,farooq2021advances, bragg2019sign, fang2017deepasl} lack a crucial element: the ability to convey emotional information in the translated text or speech. Emotional expression is vital for communication, as it helps people connect, improve relationships, and share information through dynamic, multimodal signals (e.g., visual, auditory, and spatial-temporal cues) \cite{wehrle2000studying}. As a result, hearing individuals often rely on the signer's facial expressions or context to interpret emotions. However, understanding context requires processing multiple translated sentences, making it difficult for hearing individuals to instantly grasp emotions from single-sentence-based translation systems \cite{fang2017deepasl, tanzer2024reconsidering}. This increases their reliance on interpreting facial expressions based on their own ability.

%sign language machine translation (MT) is framed as a sentence-level task. 
However, interpreting a signer’s emotions presents challenges for hearing individuals. Emotional facial expressions are inherently complex and diverse  \cite{elliott2013facial}, making it difficult for non-signing hearing people to consistently recognize the emotions. Studies have explored how hearing individuals identify signers' emotions using static \cite{creed2008psychological} or dynamic facial stimuli, achieving 78.1\% accuracy across six emotions (anger, disgust, fear, happiness, sadness, and surprise) \cite{rodger2021recognition}. However, these studies have not examined facial expression recognition alongside understanding the meaning of signs from translated information. In more realistic communication scenarios, non-signing hearing individuals need to interpret both the signer's message (via subtitles or speech) and their emotional facial expressions. This dual task potentially increases cognitive load compared to interpreting facial expressions alone, negatively impacting emotional recognition performance.

Moreover, the multifunctional use of facial expressions in sign language can make it harder for hearing individuals to interpret a signer's emotional state. Signers use facial expressions not only to convey emotions  \cite{adolphs2002recognizing} but also to fulfill various linguistic roles  \cite{shaffer2018exploring, huenerfauth2011evaluating}. For example, the linguistic marker 'INTENSE' (see below Figure \ref{fig:facialexpression} in Linguistic Markers), which indicates heightened emotions or strong emphasis, may be misinterpreted as a negative emotional expression by hearing individuals. Even when a signer is in a neutral emotional state, the hearing individual might mistakenly perceive them as angry. Additionally, when both [happy] emotions and [INTENSE] facial expressions are used—such as in the sentence "It's snowing a ton in New York" (signed as 'HERE NEW-YORK [Happy] SNOW [INTENSE]')—it can become even more difficult for hearing individuals to discern the intended emotion. Despite these challenges, no study has yet explored how hearing individuals recognize linguistic facial expressions as emotions, and also what happen on their recognition performance when linguistic markers and facial expressions are  used sequentially in a sentence. 

Additionally, current translation systems produce a neutral voice tone \cite{kahlon2023machine}, regardless of the signer's emotional state. This mismatch between voice tone and facial expressions can make it difficult for hearing individuals to accurately interpret the signer's emotions. Research on agents has shown that mismatches between voice tone and facial expression create cognitive dissonance for hearing individuals \cite{nass2001does}, negatively impacting the agent. Therefore, consistency between facial expressions and voice is crucial for effective communication, as it aids in accurate recognition of emotions. Previous research \cite{song2018gesture} incorporated emotional facial expressions into a translation system and evaluated how well synthesized emotional speech conveyed emotions. However, it remains unclear how emotional voice assists hearing individuals in recognizing a signer’s emotional state, particularly when multiple facial expressions are used for both emotions and linguistic markers.

To address these unexplored areas, this paper investigates: 
\begin{itemize}
  \item How do non-ASL hearing individuals recognize signers’ emotions when observing both
emotional facial expressions and translation information in a communication scenario?;
  \item How do non-ASL hearing individuals recognize signers’ emotions when observing linguistic
facial expressions of a signer?;
  \item How do non-ASL hearing individuals recognize signers’ emotions when observing multiple facial
expressions such as both emotional and linguistic facial expression simultaneously during signing?;
\item How should emotional voice be designed for emotional-voice translation systems to aid communication between hearing and Deaf or Hard of Hearing individuals?
\end{itemize}

We conducted an online survey with 45 participants, where respondents identified the signer's seven emotions (i.e., neutral, happy, sad, angry, terrified, disgust, and surprised) under three conditions: translated sign language text provided with no voice (only subtitles), neutral voice, and emotional voice. Additionally, we gathered open-ended feedback on the design of emotional voices from 8 DHH users and 45 hearing individuals. In the following section, we explain how we designed the experiment and survey, then report the results, and discuss the design implications of emotional voice for ASL translation systems. 

%The findings show that hearing non-ASL individuals struggle to recognize the seven emotions when signing with multiple facial expressions. Emotional voice, particularly in negative emotional states (e.g., terrified), helped improve emotion recognition. In this paper, we present a detailed analysis of these findings and provide design recommendations for emotional voice in translation systems

%  these challenges to read emotional status of signers, 

% we propose the concept of an AI generated emotional voice translator and aim to investigate its potential impact on the emotional recognition ability of hearing individuals

% Moreover, facial expressions in sign language serving multifaceted purposes might make harder for hearing people to understand their emotional status. Signers use facial expression to not only convey emotions but also fulfill various linguistic functions. For instance, the linguistic marker 'INTENSE' (see below in Linguistic Markers), which signifies heightened emotions or strong emphasis, may appear as a negative emotional expression from the perspective of hearing individuals. So, even though the signer did not express any emotions (neutral emotonal status), the hearing individual might misintpreste their emotions as negative such as angry. In additon,  when both happy emotions and 'INTENSE' facial expressions are used, such as in the sentence 'It's snowing a ton in New York' (signed as 'HERE NEW-YORK SNOW'), it may pose difficulty for hearing individuals to discern the intended emotion. However, none of studies have not yet exprelored the recognition emotion including neutral emotional status under use of lingustic facial . 

%Since emotional expression is important for communication because it helps people connect with others, improve relationships, and convey information. The facial expression of emotion is represented via dyamic multimodal signals (e.g., visual, auditory, and other spatitial-tmoporal contetual informpation). 



% Sign-to-speech translator systems help hearing individuals understand signed languages such as American Sign Language (ASL). However, current translator systems lack crucial elements necessary for generating speech, such as emotional voice tone, resulting in the production of only neutral voices. Sign language relies on facial expressions as indicators of emotional states, yet these translator systems do not integrate facial expressions to produce corresponding emotional voices. Consequently, hearing individuals have discerned emotional states either by interpreting the conversation's context or by observing the signer's emotional facial expressions. 

% However, interpreting a signer's emotions poses challenges for hearing individuals. Emotional facial expressions are intricate and diverse, making them difficult to readily recognize. Studies have shown that hearing individuals can successfully identify five emotions conveyed by signers at a rate of 63.3\%. 


% Moreover, facial expressions in sign language serve multifaceted purposes. They not only convey emotions but also fulfill various linguistic functions. For instance, the linguistic marker 'INTENSE' (see below in Linguistic Markers), which signifies heightened emotions or strong emphasis, may appear as a negative emotional expression from the perspective of hearing individuals. Consequently, when both happy emotions and 'INTENSE' facial expressions are used, such as in the sentence 'It's snowing a ton in New York' (signed as 'HERE NEW-YORK SNOW'), it may pose difficulty for hearing individuals to discern the intended emotion. 

% Additionally, current translator systems produce a neutral voice tone regardless of the signer's emotion. This lack of emotional tone alignment with facial expressions can make it challenging for hearing people to accurately interpret the signer's emotions. When there's a mismatch between the voice tone and the facial expression, it often leads to cognitive dissonance for the hearing individuals. To tackle these challenges, we propose the concept of an AI generated emotional voice translator and aim to investigate its potential impact on the emotional recognition ability of hearing individuals

% To evaluate our concept, we conducted an online survey where hearing respondents were asked to recognize the emotional status of signers by watching video clips. In these clips, signers displayed various facial expressions for both seven emotions and seven linguistic markers in ASL. 


% Many research work on recognizing facial expression only, but in real-realistic scnearion, non-hearing people need to understandin what the signer's say from the translator. in this case, the hearin people need  tod 


% facial expression of emotion are percieved dynamically with multimodal sensory information. It is unclear how facial expressions are recognized when multiple facial expression are used by signers for emotion and lingustic markers. Few studies have investigated facial expression recognitin in non asl hearing using dynamic stimuli while signing, and none have included all six basis facial expressions of emotion with neutral status (e.g., anger, disgust, happy, sad, terrified, and surprised,) with stimuli fully controlled acomppyanying with 6 lingustic markers. 

% A sign-to-speech generator translator system assists hearing individuals who are not familiar with sign language in understanding the meaning of signs. However, the lack of emotional speech from the voice generator may cause confusion for hearing individuals in comprehending the nuanced emotional meanings of translated signs, as interpreting the emotional facial expressions of signers can be difficult for them. For instance, hearing people often find it confusing, particularly when ASL linguistic markers coincide with emotional facial expressions. Additionally, mismatched voice and facial expressions can further confuse hearing individuals, leading to cognitive dissonance. For example, neutral translated voice speech following ‘sad’ facial expressions from the signer can confuse hearing people. 

% In this study, we explore the significant impact of an emotional voice translator on improving hearing people’s understanding of the emotional status of signers in translated signs. 

% "NEED - explain scenarios"

% Contribution 
% - first evaluation on how emotional voice is necessary of sign-to speech translator for hearing people. 

% assumption

% meaning is delivered by translator, but the emotional status should be read by hearing people to get sense of translated sign.

% 1. we assume that hearing people can understand facial expression for emotional status. 
% 2. 


% \subsection{the importance of emotional voice for communication}
% Emotional communication is an important part of social interaction because it gives individuals valuable information about the state of others, allowing them to adjust their behaviors and responses appropriately \cite{nordstrom2019emotional}. 



==> document/03_research_question.tex <==
\section{Research Questions}
Based on the analysis of previous work, there is a discrepancy in understanding how hearing people recognize a signer’s emotional state, especially when the signer uses multiple facial expressions as both linguistic markers and indicators of emotion. Additionally, due to cognitive dissonance, current sign-to-speech translation systems may cause confusion for hearing individuals since the "neutral" voice does not align with the signer’s facial expressions. To address these issues, we believe that emotional voices should be integrated into sign-to-speech translation systems. Our research questions fall into two categories: RQ1: How can emotional voices in the translation systems help non-ASL hearing individuals recognize a signer’s emotions? RQ2: How have emotional voices in the system been designed for both DHH users and hearing individuals?



In this paper, we explore the sub-research questions under RQ1 and RQ2:
\begin{itemize}
  \item RQ1-1: How do non-ASL hearing individuals interpret linguistic facial expressions as emotions?
  \item RQ1-2: How can hearing individuals recognize a signer’s emotional state by interpreting facial expressions when multiple expressions, such as grammatical and linguistic markers, are used?
  \item RQ1-3: How do hearing individuals experience confusion when a neutral voice is generated, regardless of the signer’s emotions?
  \item RQ1-4: How can emotional voices help hearing individuals understand a signer’s emotions when multiple expressions are used?
  \item RQ2-1: How has the emotional voices been designed for users (non-ASL hearing and DHH individuals)?
  
\end{itemize}



%   \item 1) RQ1: How do non-ASL hearing individuals recognize signers’ emotions when observing both
% emotional facial expressions and translation information in a communication scenario?;
%   \item 2) RQ2: How do non-ASL hearing individuals recognize signers’ emotions when observing linguistic
% facial expressions of a signer?;
%   \item 3) RQ3: How do non-ASL hearing individuals recognize signers’ emotions when observing multiple facial
% expressions such as both emotional and linguistic facial expression simultaneously during signing?
% \item 4) RQ4: How should emotional voice be designed for emotional-voice translation systems to aid
% communication between hearing and Deaf or Hard of Hearing individuals?

==> document/05_result.tex <==
\section{Result}
In this section, we analyzed the data in two categories: the use of single facial expressions and multiple facial expressions. For each category, we conducted a between-subjects analysis as follows: Condition A: 14 responses (age range: 19 to 29, mean: 21.29, SD: 3.12, male: 4, female: 10); Condition B: 15 responses (age range: 18 to 43, mean: 22.73, SD: 6.68, male: 6, female: 9); Condition C: 15 responses (age range: 19 to 33, mean: 21.76, SD: 3.96, male: 4, female: 12) 



\subsection{Single Facial Expression: Emotion Only}
We explored the difference in recognition performance when reading facial expressions alone versus reading both the emotions and meaning of the sign. We also examined how non-ASL hearing individuals understood emotional facial expressions under three conditions, focusing on instances where the signer used only a single facial expression to convey emotion.

\subsubsection{Recognition of Emotion: With or Without Signing}

We hypothesized that recognizing emotions while interpreting the meaning of signs is more challenging than reading facial expressions alone. There is a significant difference in recognition performance between the two conditions. When participants only read facial expressions, they achieved an accuracy of 80.19\% (SD: 19.54\%) with a cognitive load of 2.90 (SD: 1.78). However, recognition accuracy while signing was lower across three conditions: 31.12\% (SD: 14.18\%) for Condition A, 33.81\% (SD: 12.21\%) for Condition B, and 46.67\% (SD: 11.73\%) for Condition C. The cognitive load for the three conditions was 3.12 (SD: 1.05), 4.60 (SD: 1.09), and 3.04 (SD: 1.32), respectively. Understanding the meaning of signs showed performance levels of 86.71\% (SD: 11.55\%), 91.90\% (SD: 2.51\%), and 91.43\% (SD: 2.96\%) with cognitive load values of 1.56 (SD: 0.86), 4.74 (SD: 2.38), and 1.16 (SD: 0.28), respectively. Our findings suggest that the dual task of understanding both the meaning of the signs and the emotions increases cognitive workload, negatively impacting emotion recognition performance.

% This is because the cognitive workload increases when individuals need to both interpret the signer's message and recognize their emotions. 

\begin{figure}
    \includegraphics[width=1\linewidth]{document//figures/emo_only.png}
    \caption{Recognition of Emotion: With or Without Signing Using a Single Facial Expression}
    \label{fig:enter-label}
\end{figure}
\subsubsection{Comparison of Recognition Performance Across Three Conditions}
We hypothesized that emotional voice can help hearing individuals better understand a signer’s emotional state. The results showed that providing emotional voice improved recognition performance by 13–15\%, achieving 46.67\% accuracy compared to the other two Conditions A and B. When the corresponding emotional voice was provided alongside the signer’s emotional state, it helped hearing participants recognize stronger or negative emotions (e.g., angry, sad, surprised, terrified) more effectively than neutral or positive emotions (see confusion matrix \ref{single-facial-emotion}).
Interestingly, across all three conditions, many responses misclassified emotions as "neutral" or "sad." Participants tended to perceive the signer’s neutral emotional state as "sad," with 25\% and 47\% of responses in Conditions B and C, respectively. We hypothesized that this may be due to participants being exposed to longer durations of neutral facial expressions compared to the brief emotional expressions, which lasted about one second. If the emotional expression, such as a smile for "happy," was not sufficiently striking, participants may have defaulted to perceiving it as neutral. 


% In addition to the overall recognition accuracy, participants' performance for each individual emotion also declines when transitioning from facial expressions alone to facial expressions combined with signing. When only emotional facial expressions are presented, recognition performance is generally high, with the highest accuracy for \textit{sad} at 96\% and the lowest for \textit{angry} at 56\%. These results establish that people perform well in recognizing emotions based solely on facial expressions. This is likely because focusing on a single task reduces cognitive workload, leading to better overall performance.

% Under condition A, participants were present with subtitles and facial expressions at the same time. According to our hypothesis, this dual task might impose a greater cognitive workload, affecting participants' ability to accurately recognize emotions and interpret the signers' messages. 

% The confusion matrix reveals a significant pattern of emotions being misinterpreted as neutral under condition A, with happy and sad showing the highest confusion rates at 57\% each. In comparison to the baseline condition, recognition performance in condition A deteriorates for all emotions, including neutral. This decline may be attributed to the need to divide attention between both subtitles and facial expressions, especially when these elements are visually separated. The divided focus can lead to decreased sensitivity to subtle variations in facial expressions, reducing the accuracy of emotional perception. Additionally, since the ASL sentences are crafted to convey neutral emotions without strong emotional expressions, participants may perceive the overall conveyed emotion as neutral.

% Under condition B, where participants were aided by a neutral voice for message interpretation, overall performance improved by 8.64\%. In contrast to condition A, where hearing participants relied on subtitles for message comprehension, the addition of voice assistance allowed them to focus more on facial expressions and signing while simultaneously processing the message through auditory cues. This reduction in visual workload likely enabled participants to make more detailed observations, leading to a more accurate identification of the emotions conveyed through facial expressions.E motions that showed marked improvement with neutral voice assistance included sad, surprised, and terrified, with increases of 62.07\%, 104.76\%, and 48.28\% respectively. In contrast, recognition performance for the neutral emotion declined by approximately 45.9\%, while the recognition of other emotions remained relatively stable.

% Condition C achieved the highest accuracy of 46.67\% in the group with signing. In comparison to conditions A and B, condition C demonstrated superior performance across nearly all emotions, with the exception of "happy." The most pronounced improvements were observed in the recognition of "surprised" and "terrified," both reaching 60\% accuracy. These findings highlight the critical role of emotional voice in enhancing emotion recognition among hearing participants, particularly for negative emotions. Notably, recognition of the positive emotion "happy" showed no improvement from condition B to C and even declined by 1\% from A to C. In contrast, negative emotions such as "angry," "disgust," "sad," and "terrified" exhibited varying levels of improvement, with the most significant increase observed for "angry," which rose by 115\% from B to C and 104.76\% from A to C. This indicates that emotional voice support has a more substantial impact on the recognition of negative emotions than positive ones.

\begin{figure}[H]
    \includegraphics[width=1\linewidth]{document//figures/only_e_cm.png}
    \caption{Confusion Matrix for Recognition Performance of Single Facial Expression: Emotion Only}
    \label{fig:single-facial-emotion}
\end{figure}


% \subsubsection{Mismatched Voice and Matched Facial Expression}
% We hypothesized that the absence of emotional vocal tones in the current system might create a cognitive dissonance due to the mismatch between a neutral voice and emotional facial expressions. Consequently, we sought to examine whether this incongruence would make it more challenging for hearing individuals to accurately identify the intended emotions.

% Contrary to our hypothesis, the results revealed that the addition of a neutral voice actually improved emotion recognition accuracy by 2.69\% from condition A to condition B. A possible explanation for this could be the distraction caused by subtitles in condition A, which may have shifted participants' focus away from facial expressions. In contrast, when voice assistance was provided in condition B, hearing individuals were better able to concentrate on facial cues, thereby improving their ability to recognize emotions.

\subsection{Single Facial Expression: Linguistic Marker Only}
Non-ASL hearing individuals are generally not aware of linguistic facial expressions, and they may recognize these linguistic markers as emotional states. We explored how non-hearing individuals perceived linguistic markers as emotions and whether correlating emotional voices, i.e., 'neutral' voice tone can aid their understanding of 'neutral emotion'. 
% We explore the difference in recognition performance when reading facial expressions alone versus reading both the emotion and meaning of the sign. We also examine how hearing non-ASL individuals understand emotional facial expressions under three conditions, focusing on instances where the signer uses only a single facial expression to convey emotion.
\subsubsection{Linguistic Marker Considered as Emotions}
Participants were asked to select an emotion based on only the facial expressions (without signing) associated with linguistic markers. The results showed that linguistic markers were most commonly misinterpreted as 'disgust.' Specifically, TH, INTENSE, CS, and PS were perceived as 'disgust' at rates of 91\%, 84\%, 78\%, and 44\%, respectively. Additionally, MM and PUFF were perceived as 'sad' by 31\% and 40\% of participants. Interestingly, PS was perceived as 'happy' by 27\%. Overall, linguistic markers were interpreted as conveying negative or intense emotions, suggesting that these markers could give the impression of strong or negative emotional expression, potentially leading to misunderstanding by non-hearing individuals during conversations.
However, differences in perception emerged between signing and non-signing scenarios. Participants recognized the signer's emotions as neutral with about 40\% to 52.25\% accuracy, despite being able to observe linguistic facial expressions while signing. It was possible that these facial expressions were too subtle or brief, leading respondents to select neutral emotions. Stronger facial expressions associated with linguistic markers, such as INTENSE and PUFF, were still perceived as 'angry' or 'disgusted,' while less distinct linguistic facial expressions, like MM, CS, and TH, were commonly interpreted as 'sad' across the three conditions (See Confusion Matrix \ref{fig:single-facial-linguistic}).The results showed no difference in recognition performance of the 'neutral' emotion across the three conditions (stat). All conditions followed similar patterns, where slightly stronger facial expressions were perceived similarly.

% % include perceiving MM to be sad 40\%, and PUFF to be sad 31\% of the time and so on. 



% such as INTENSE, PUFF, 

% % Among all linguistic markers, INTENSE and PUFF are mostly perceived to be negative emotion angry with the percentage to be 40.5\% and 38.6\%  separately. Other common mappings are MM with sad (20.0\%), CS with sad (20.5\%), TH with disgusted (17.1\%), PS with angry (20.0\%). The tendency of categorizing lingusitic markers to be emotions causes confusion among non-ASL hearing people about the signer's emotional state.

%  Additionally, there is a notable difference between recognizing facial expressions alone and interpreting them with signing, highlighting that non-ASL hearing people struggle more when facial expressions are combined with signing. The results show that when only observing facial expressions with linguistic markers, the perceived accuracy is lower than the condition with emotional facial expression only. Nevertheless, the performance is better than the case when linguistic markers combined with neutral voice. When only the neutral voice is paired with linguistic markers, it is more difficult for hearing people to find clues for emotions given that they don't have enough experiences with understanding linguistic markers and the neutral voice, in this case, becomes a barrier when occurring simultaneously with facial expressions with linguistic markers.
% % \begin{figure}[H]
% %     \centering
% %     \includegraphics[width=0.5\linewidth]{document//figures/only_lin_bar.png}
% %     \caption{Linguistic Marker Only}
% %     \label{fig:enter-label}
% % \end{figure}

% As a baseline for recognition performance, we presented linguistic facial expressions without signing to participants. The results indicate that CS, INTENSE, and TH elicited a strong association with specific emotions, while MM, PS, and PUFF resulted in relatively even perception across multiple emotions. Specifically, TH exhibited the highest confusion rate with disgust, at 91\%. Similarly, INTENSE and CS had high confusion rates with disgust, at 78\% and 84\%, respectively. MM was perceived as sad, neutral, and surprised, with confusion rates of 40\%, 29\%, and 22\%, respectively. PS was associated with disgust, happiness, and neutrality, with confusion rates of 44\%, 22\%, and 16\%, respectively. PUFF was primarily perceived as sad and disgusted, with confusion rates of 31\% and 29\%, respectively.


\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{document//figures/lin_only.png}
    \caption{Linguistic Marker Only}
    \label{fig:Linguistic Marker Only Confusion Matrix}
\end{figure}

% Under condition A, where signing was integrated into the perception process and subtitles were added to assist interpretation, the overall perceptions of linguistic markers were inclined to align with neutral emotion with the average confusion score to be 52.57\% . Specifically, PS, TH, MM, CS, and PUFF each had their highest confusion scores associated with the neutral emotion, at 71\%, 61\%, 54\%, 46\%, and 46\%, respectively.

% Additionally, CS was also perceived as sad, with a confusion score of 39\%, and MM was similarly perceived as sad, with a confusion score of 43\%.

% Under condition B, the overall trend remains consistent, with most linguistic markers still being perceived as neutral. However, the average confusion score decreases to 40\%. Notable changes occur when linguistic markers are paired with neutral voice: INTENSE is predominantly perceived as disgusted, with a confusion score of 53\%; NONE is predominantly perceived as sad, with a confusion score of 47\%; and TH is predominantly perceived as disgusted, with a confusion score of 30\%.

% Under condition C, where emotional voice was provided, the overall perception of linguistic markers once again concentrated on neutral emotions, with an average confusion score of 51.57\%. This score is similar to the average score observed under condition A.


% \subsubsection{emotional voice help?}
% Previous results suggest that linguistic markers are frequently mistaken for emotions, causing communication challenges between hearing and deaf individuals. We hypothesized that introducing a neutral voice might help disambiguate emotions. However, the results indicated the opposite. When the test sample was limited to linguistic markers alone, conditions B and C, both employing neutral voice, effectively presented the same test to participants. Despite this, performance in conditions B and C was lower than in condition A, with a mean accuracy of 0.46—13\% lower than that of condition A.

% We posit that one potential explanation is the contrast between the neutral voice and the facial expressions with the linguistic markers. Hearing participants may experience cognitive dissonance when attempting to interpret the overall emotion, as they form conflicting perceptions based on the audio and facial expressions, leading to greater confusion in some cases.


\begin{figure}[H]
    \includegraphics[width=1\linewidth]{document//figures/only_lin_cm.png}
    \caption{Confusion Matrix for Recognition Performance of Single Facial Expression: Linguistic Marker Only}
    \label{fig:single-facial-linguistic}
\end{figure}



\subsection{Multiple Facial Expressions: Emotion and Linguistic Marker}
In this section, we explore how non-ASL hearing individuals recognize a signer’s emotions when observing multiple facial expressions associated with linguistic markers and emotions. First, we examine hearing individuals' recognition abilities across three conditions, followed by an analysis of the effect of the order in which facial expressions are presented.

\subsubsection{Comparison of Recognition Performance Across Three Conditions: Mulitple Facial Expression}

We hypothesized that emotional voice can effectively enhance the perception of emotions among non-ASL hearing individuals. The results indicated that the impact of emotional voice varies across emotions, with a notable enhancement observed in five out of seven emotions. A comparison across the three conditions demonstrated a significant improvement in performance when emotional voice was present for surprised, terrified, angry, sad, and disgusted emotions. Among these, surprised and terrified showed the most pronounced enhancement. Specifically, the recognition accuracy for surprised increased by 186.36\% compared to condition A and by 75\% compared to condition B. Similarly, recognition accuracy for terrified improved by 104.76\% compared to condition A and by 65.38\% compared to condition B. On the contrary, our emotional voice system yielded approximately the same performance with condition A for neutral and worse performance with condition B for happy.

% reasons why enhancement in those particular emotions and decrease in neutral and happy


The results suggested that emotional voice played a critical role in enhancing recognition performance, particularly in cases where facial expressions are mistakenly perceived as neutral. A comparison of the confusion matrices under conditions A, B, and C revealed that, with the addition of emotional voice, the misclassification of emotions as neutral decreases significantly, leading to a stronger alignment with the intended emotions. More specifically, the misclassification rate of emotions with neutral decreases 48.36\% on average for sad, angry, terrified, surprised and disgusted compared with condition A and 52.04\%  compared with condition B.




\begin{figure}[H]
    \centering
    \includegraphics[width=0.6\linewidth]{document//figures/rp_conditions.png}
    \caption{Recognition Performance by Conditions}
    \label{fig:enter-label}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{document//figures/perf_all.png}
    \caption{General Recognition Performance}
    \label{fig:enter-label}
\end{figure}



\subsubsection{Confusion Matrix When Emotional Voice Provided}

Based on the analysis of the overall confusion matrix and an examination of recognition performance across combinations of facial expressions and linguistic markers, we propose two key hypotheses:

\begin{enumerate}
    \item When both emotions and linguistic markers are misclassified, the combination leads to a higher overall confusion rate, particularly for misunderstood emotions.
    \item The intensity and duration of emotions influence perception patterns. Specifically, we suggest the following:
    \begin{itemize}
        \item Emotions with lower intensity and shorter duration are more susceptible to the influence of misclassification of linguistic markers.
        \item If linguistic markers are misclassified as emotions with greater intensity and longer duration, their influence on perception becomes more pronounced.
        \item When an emotion with lower intensity and shorter duration is paired with a linguistic marker misclassified as an emotion with higher intensity and longer duration, the confusion rate increases significantly.
    \end{itemize}
\end{enumerate}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{document//figures/cm_complete.png}
    \caption{Complete Confusion Matrix}
    \label{fig:enter-label}
\end{figure}

The combination of "happy" with the linguistic marker "TH" demonstrates the lowest recognition performance. When emotional voice is present, "happy" exhibits a confusion rate with "neutral" of 0.57. Similarly, "TH" is consistently misclassified as "neutral" at a rate of 0.305. In contrast, when "happy" is paired with other linguistic markers, performance improves and the confusion with "neutral" decreases. For example, when paired with "PUFF," which is frequently misclassified as "angry" (38.6\%), recognition accuracy reaches 0.49, and the confusion rate with "neutral" falls to 0.32. However, when "happy" is paired with "TH," the confusion rate with "neutral" rises to 0.43, and recognition accuracy drops to only 0.15. This combination intensifies the misinterpretation of both "happy" and "TH" as "neutral," further confusing participants, who tend to categorize the emotion as "neutral" due to the overlapping misclassification.

Overall, recognition performance is higher for "angry" and "sad," with recognition accuracy of 0.56 and 0.54 respectively, and lower for "terrified" and "disgusted," both at 0.43. This variation can be attributed to the intensity and duration of emotions. Prior research \cite{brans2014intensity} has shown that "sadness" and "anger" exhibit greater intensity and longer duration, while "disgust" is characterized by the lowest intensity and shortest duration. "Fear" (terrified) is also noted for its shorter duration.

To further illustrate our hypotheses, we examined combinations with the lowest recognition accuracy. Emotions with low intensity and short duration are more prone to be influenced by the misclassification of linguistic markers. The combination of "disgusted" with "CS" is frequently perceived as "neutral" (34\%) or "happy" (39\%). Although "disgust" generally performs well, "CS" is typically misclassified as "neutral" (30.0\%) or "happy" (12.9\%). Given that "disgust" has the lowest intensity and shortest duration, it aligns with our hypothesis that it is more susceptible to the influence of misclassified linguistic markers. Consequently, recognition of this combination is dominated by how "CS" is perceived rather than "disgust." In comparison, "angry," which is higher in intensity and longer in duration, remains more accurately recognized, achieving a recognition accuracy of 0.42, compared to 0.16 for the combination of "disgust" with "CS."

When linguistic markers are misclassified as emotions with higher intensity and longer durations, their impact on perception increases significantly. For instance, the combination of "happy" with "INTENSE" is predominantly perceived as "neutral" (0.31\%) or "angry" (0.25\%). "INTENSE" aligns most closely with "angry," with a recognition accuracy of 0.77, suggesting a strong alignment between the two for hearing people. The intensity and duration of "angry" exert a powerful influence, causing participants to misinterpret the emotion as "angry," leading to confusion and a tendency to select "neutral" or "angry."

Finally, when an emotion with lower intensity and shorter duration is paired with a linguistic marker misclassified as an emotion with higher intensity and longer duration, confusion rates increase substantially. For example, when "terrified," which has moderate intensity but shorter duration, is paired with "PUFF," which is misclassified as "angry" (high intensity and long duration), recognition accuracy drops to 0.08, with a 0.64 confusion rate for "angry."



\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{document//figures/cmA.png}
    \caption{Confusion Matrix - A}
    \label{fig:enter-label}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{document//figures/cmB.png}
    \caption{Confusion Matrix - B}
    \label{fig:enter-label}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{document//figures/cmC.png}
    \caption{Confusion Matrix - C}
    \label{fig:enter-label}
\end{figure}





\subsection{Order: EL vs LE}
Overall, recognition performance is higher when the sequence follows linguistic markers before emotions, with an accuracy of 0.42, compared to 0.365 when the order is emotions before linguistic markers.

However, this effect of order varies across emotions under the three conditions. The recognition accuracy is consistently greater for happy and sad emotions when the order is linguistic markers before emotions across all conditions. For other emotions, performance varies depending on the order. Therefore, although the linguistic markers → emotions order results in better overall performance compared to the reverse, the order does not appear to play a decisive role in emotion perception.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{document//figures/order_1.png}
    \caption{Overall Recognition Performance by Order}
    \label{fig:enter-label}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{document//figures/order_2.png}
    \caption{Recognition Performance by Order}
    \label{fig:enter-label}
\end{figure}


\subsection{Features}

To further explore the design implications for hearing individuals, we included an open-ended question about additional features or characteristics of emotional voice that require attention when designing the translation system. In total, we received 43 responses from hearing individuals and 6 responses from DHH individuals.

For hearing participants, pitch was highlighted in 11 responses as the most emphasized property for detecting emotional cues, with volume and intensity contributing to the expression of emotional strength. One participant noted that pitch is often the most effective indicator of specific emotions and serves as a critical cue for hearing individuals to identify emotions. Intensity and volume were also emphasized in 8 and 7 responses, respectively.

There were also concerns about AI-generated voices sounding too robotic or lacking natural inflection. Two participants pointed out that AI voices should sound more human-like, with nuanced variations in pitch and tone, to avoid discomfort and improve communication clarity. Additionally, nine hearing participants stressed the importance of making the tone more natural and personalized to better resemble human emotional expression.

The DHH group mainly emphasized on the importance of intensity of the voice and natural tone. One participant contended that, "Intensity and tone would be good since deaf people’s ASL can vary in tone and intensity by their emotions and is something in every conversation."

In the open-ended question, we also asked participants whether the seven emotions provided in the study were sufficient for simulating human emotional voice. Among the hearing participants, only ten felt that the emotions were sufficient, while the majority believed that more emotions were needed or that some of the provided emotions were unclear. Common suggestions for additional emotions included anxious, disappointed, satisfied, speechless, and bored. Several participants also noted the lack of positive emotions.

One participant emphasized the deeper meaning behind conveyed emotions, stating, "I kept thinking 'she looks bored' during the survey and ended up choosing 'neutral' or 'sad' for many of them. These seven basic emotions are fine, but they fail to convey deeper meaning. For example, there's a difference between being glad and being ecstatic." This suggests that future designs could incorporate more contextual elements to better convey the nuances and depth of emotional expression.

For DHH participants, only one felt that the seven emotions were sufficient. Others highlighted the multidimensional nature of emotions, with one participant stating, "I don't think 7 emotions are sufficient. Emotion is complex and should be viewed as a spectrum with multiple dimensions."

% \subsection{How do hearing individuals recognize a signer’s emotions when multiple facial expressions, including linguistic markers, are used?}


 
\subsection{Importance Ranking of Emotions}

We collected data from 7 DHH participants and 43 hearing participants to assess the importance ranking of different emotions for the emotional voice ASL translation system. Negative emotions, such as anger, fear (terrified), and sadness, were consistently ranked higher than positive emotions. Both DHH and hearing participants identified angry as the most important emotion to recognize, while neutral emotion was ranked as the least important. Happy was ranked as the second most important emotion for the DHH group but ranked the second least important in the hearing group. At the same time, other emotions' rankings were similar between the two groups.

Participants emphasized that negative emotions are often associated with urgent or intense situations where individuals may face physical or psychological harm, sending signals to warn others or seek help. One hearing participant emphasized that "Negative emotions require more careful reactions from the listener, so it is critical for the receiver of the message to know what they are facing." Another DHH participant stated that, "Obviously negative emotions should be detected as soon as possible because it affects the safety of your situation. And people can be hurt with negative emotions."

\textit{Happy} was perceived differently between the DHH and hearing groups. Among DHH participants, \textit{happy} was frequently noted as a highly popular and commonly expressed emotion in American Sign Language. Due to its prevalence, many DHH participants considered it crucial for daily conversations, as accurately conveying happiness helps ensure smooth communication. Some participants also mentioned that \textit{happy} could be used interchangeably with other emotions, such as \textit{surprised}, depending on the context. This highlights the importance of recognizing \textit{happy} not just as an isolated emotion, but one with versatile usage in the DHH community.

On the contrary, positive emotions, especially among hearing participants, were considered easier to recognize and less likely to lead to serious consequences if misunderstood, underscoring the need to prioritize the detection of negative emotions. Participants also emphasized the importance of first distinguishing between polarized emotions, such as \textit{angry} and \textit{happy}, as these tend to be more extreme and easier to express. In contrast, emotions that are less intense or more subtly conveyed were generally considered less important by comparison.

